Detection of Partially Visible Objects

An "elephant in the room" for most current object detection and localization methods is the lack of explicit modelling of partial visibility due to occlusion by other objects or truncation by the image boundary. Based on a sliding window approach, we propose a detection method which explicitly models partial visibility by treating it as a latent variable. A novel non-maximum suppression scheme is proposed which takes into account the inferred partial visibility of objects while providing a globally optimal solution. The method gives more detailed scene interpretations than conventional detectors in that we are able to identify the visible parts of an object. We report improved average precision on the PASCAL VOC 2010 dataset compared to a baseline detector.

==> res_occmod_nms_table.tex <==
\begin{table}
  \center
 \begin{tabular}{| >{\centering\arraybackslash}m{75pt} | 
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 									 >{\centering\arraybackslash}m{35pt} |
 								}
 %\begin{tabular}{|c||c|c|c|c|c|c|c|}
	\hline
   AP (on {\texttt{\footnotesize{test}}})	
				& 		aero & 		bicycle & 		bird & 		boat & 		bottle & 		bus & 		car \\
   \hline
   \emph{VIS}		& 	 \pv{27.7} & 	    	27.7 & 		0.1 & 		3.2 & 		1.0 & 		31.9 & 		22.9 \\
   \emph{VIS+NMS}	& 	 	26.3 &	 \pv{28.1} & 		0.1 & 		3.2 & 		1.0 &	 \pv{32.5} &	  \pv{23.7} \\
   \hline \hline
   AP (on {\texttt{\footnotesize{test}}})	
				& 		cat & 		chair & 		cow & 		table & 		dog & 		horse & 		person \\
   \hline
   \emph{VIS}		& 		3.0 & 		5.6 & 		5.2 & 	 \pv{4.9} & 		3.9 & 	 \pv{14.4} & 	 \pv{16.2} \\
   \emph{VIS+NMS}	& 		3.0 &	 \pv{5.8} &	 \pv{5.3} &		4.3 &		3.9 &		13.7 &		15.8 \\
   \hline \hline
   AP (on {\texttt{\footnotesize{test}}})	
				& 		mbike & 		plant & 		sheep & 		sofa & 		train & 		tv & 			mean \\
   \hline
   \emph{VIS}		& 		27.1 & 		3.5 & 	 \pv{7.8} & 	 \pv{3.3} & 	 \pv{12.8} & 	 \pv{26.9} & \textbf{\textit{12.5}} \\
   \emph{VIS+NMS}	& 	 \pv{27.2} &		3.5 &		7.5 &		3.2 &		12.2 & 		25.9 & 		12.3 \\
   \hline 
  \end{tabular}
  \caption[AP results for PASCAL VOC 2010 (partial visibility modeling) II]{PASCAL VOC 2010 results ({\texttt{\small{comp3}}}, {\texttt{\small{test}}}-set). We show Average Precision (AP) for a models with $d=2$ mixture components at a threshold of $t=-1$. \emph{VIS} uses the greedy NMS scheme~\cite{Felzenszwalb10} while \emph{VIS+NMS} uses the globally optimal NMS scheme presented in Section~\ref{chap_occmod:sec:nms} used. AP improves for $6$ of $20$ object classes while mean AP drops slightly from $11.4\%$ to $11.3\%$ when comparing \emph{VIS} to \emph{VIS+NMS}.}
  \label{chap_occmod:tab:2010nmsres}
\end{table}
